Arduino control of a pulsatile flow rig

This note describes the design and testing of a programmable pulsatile flow pump using an Arduino micro-controller. The goal of this work is to build a compact and affordable system that can relatively easily be programmed to generate physiological waveforms. The system described here was designed to be used in an in-vitro set-up for vascular access hemodynamics research, and hence incorporates a gear pump that can deliver up to 1.5 l/min in a test flow loop. After a number of simple identification experiments to assess the dynamic behaviour of the system, a feed-forward control routine was implemented. The resulting system was shown to be able to produce the targeted patient-specific waveform with less than 3.6% error. Finally, we outline how to further increase the accuracy of the system, and how to adapt it to specific user needs.

==> DynFit_virt.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{009}[tc][tc]{\matlabtextA $t$ (s)}%
\psfrag{010}[bc][bc]{\matlabtextA virtual flow (pwm)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $10$}%
\psfrag{002}[ct][ct]{\matlabtextB $20$}%
\psfrag{003}[ct][ct]{\matlabtextB $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextB $0$}%
\psfrag{005}[rc][rc]{\matlabtextB $50$}%
\psfrag{006}[rc][rc]{\matlabtextB $100$}%
\psfrag{007}[rc][rc]{\matlabtextB $150$}%
\psfrag{008}[rc][rc]{\matlabtextB $200$}%
%
%% </ytick>

==> LinFit_resubmit.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{009}[tc][tc]{\matlabtextA $t$ (s)}%
\psfrag{010}[bc][bc]{\matlabtextA virtual flow (-)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $10$}%
\psfrag{002}[ct][ct]{\matlabtextA $20$}%
\psfrag{003}[ct][ct]{\matlabtextA $30$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextA $0$}%
\psfrag{005}[rc][rc]{\matlabtextA $50$}%
\psfrag{006}[rc][rc]{\matlabtextA $100$}%
\psfrag{007}[rc][rc]{\matlabtextA $150$}%
\psfrag{008}[rc][rc]{\matlabtextA $200$}%
%
%% </ytick>

==> MeasRefFilt.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{012}[tc][tc]{\matlabtextA $t$ (s)}%
\psfrag{013}[bc][bc]{\matlabtextA $Q$ (l/min)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $0.2$}%
\psfrag{002}[ct][ct]{\matlabtextB $0.4$}%
\psfrag{003}[ct][ct]{\matlabtextB $0.6$}%
\psfrag{004}[ct][ct]{\matlabtextB $0.8$}%
\psfrag{005}[ct][ct]{\matlabtextB $1$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextB $0.7$}%
\psfrag{007}[rc][rc]{\matlabtextB $0.8$}%
\psfrag{008}[rc][rc]{\matlabtextB $0.9$}%
\psfrag{009}[rc][rc]{\matlabtextB $1$}%
\psfrag{010}[rc][rc]{\matlabtextB $1.1$}%
\psfrag{011}[rc][rc]{\matlabtextB $1.2$}%
%
%% </ytick>

==> NonLinFit_resized.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{012}[bc][bc]{\matlabtextA $Q$ (l/min)}%
\psfrag{013}[tc][tc]{\matlabtextA $u$ (V)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\psfrag{000}[ct][ct]{\matlabtextA $0$}%
\psfrag{001}[ct][ct]{\matlabtextA $5$}%
\psfrag{002}[ct][ct]{\matlabtextA $10$}%
\psfrag{003}[ct][ct]{\matlabtextA $15$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{004}[rc][rc]{\matlabtextA $0$}%
\psfrag{005}[rc][rc]{\matlabtextA $0.2$}%
\psfrag{006}[rc][rc]{\matlabtextA $0.4$}%
\psfrag{007}[rc][rc]{\matlabtextA $0.6$}%
\psfrag{008}[rc][rc]{\matlabtextA $0.8$}%
\psfrag{009}[rc][rc]{\matlabtextA $1$}%
\psfrag{010}[rc][rc]{\matlabtextA $1.2$}%
\psfrag{011}[rc][rc]{\matlabtextA $1.4$}%
%
%% </ytick>

==> ffSig_new_resized_grid.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{012}[tc][tc]{\matlabtextA $t$ (s)}%
\psfrag{013}[bc][bc]{\matlabtextA virtual flow (pwm)}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextB{\color[rgb]{0.150,0.150,0.150}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextB $0$}%
\psfrag{001}[ct][ct]{\matlabtextB $0.2$}%
\psfrag{002}[ct][ct]{\matlabtextB $0.4$}%
\psfrag{003}[ct][ct]{\matlabtextB $0.6$}%
\psfrag{004}[ct][ct]{\matlabtextB $0.8$}%
\psfrag{005}[ct][ct]{\matlabtextB $1$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{006}[rc][rc]{\matlabtextB $-50$}%
\psfrag{007}[rc][rc]{\matlabtextB $0$}%
\psfrag{008}[rc][rc]{\matlabtextB $50$}%
\psfrag{009}[rc][rc]{\matlabtextB $100$}%
\psfrag{010}[rc][rc]{\matlabtextB $150$}%
\psfrag{011}[rc][rc]{\matlabtextB $200$}%
%
%% </ytick>
